On Algorithms and Complexity for Sets with Cardinality Constraints

Typestate systems ensure many desirable properties of imperative programs, including initialization of object fields and correct use of stateful library interfaces. Abstract sets with cardinality constraints naturally generalize typestate properties: relationships between the typestates of objects can be expressed as subset and disjointness relations on sets, and elements of sets can be represented as sets of cardinality one. Motivated by these applications, this paper presents new algorithms and new complexity results for constraints on sets and their cardinalities. We study several classes of constraints and demonstrate a trade-off between their expressive power and their complexity. Our first result concerns a quantifier-free fragment of Boolean Algebra with Presburger Arithmetic. We give a nondeterministic polynomial-time algorithm for reducing the satisfiability of sets with symbolic cardinalities to constraints on constant cardinalities, and give a polynomial-space algorithm for the resulting problem. In a quest for more efficient fragments, we identify several subclasses of sets with cardinality constraints whose satisfiability is NP-hard. Finally, we identify a class of constraints that has polynomial-time satisfiability and entailment problems and can serve as a foundation for efficient program analysis.

==> conclusions.tex <==
\section{Conclusions}

Constraints on sets and relations are very useful for
analysis of software artifacts and their abstractions.
Reasoning about sets and relations often involves reasoning
about their sizes.  For example, an integer field may be
used to track the size of the set of objects stored in a
data structure.  In this paper, we have presented new
complexity results and algorithms for solving constraints on
boolean algebra of sets with symbolic and constant
cardinality constraints.  We have presented symbolic
constraints and large constant constraints, gave more
efficient algorithm for quantifier-free symbolic
constraints, identified several sources of NP-hardness of
constraints, and presented a new class of constraints for
which satisfiability and entailment are solvable in
polynomial time.  We hope that our results will serve
as concrete recipes and general guidance in the design
of algorithms for constraint solving and program analysis.


==> preliminaries.tex <==
\smartparagraph{Preliminaries.}
If $S$ is a finite set, $|S|$ denotes the number of elements
in $S$.  A literal is an atomic formula or its negation.
$\Integ = \{ \ldots, -1, 0,1,\ldots \}$ is the set of
integers, $\Nat = \{ 0, 1, \ldots\}$ is the set of natural
numbers.  $[a..b]$ denotes the set of integers
$\{a,a+1,\ldots,b\}$.  If $f : A \to B$ is a function and $S
\subseteq A$, we define $f[S] = \{ f(a) \mid a \in S \}$.

If $A$ is a set, the notation $A^y$ has several potential meanings;
the specific meaning should be clear from the context.  $A^n$ for $n \in \{ 1, 2,
\ldots, \}$ is the set of vectors $(a_1,\ldots,a_n)$ where
$a_j \in A$ for $1 \leq j \leq n$, and $A^{m,n}$ is the set
of matrices $[a_{pq}]$ with $m$ rows and $n$ columns with
elements $a_{pq}$ for $1 \leq p
\leq m$ and $1 \leq q \leq n$.  
The expression $A^c$ denotes the complement of the set $A$.
If $\alpha \in \{0,1\}$, then $A^{\alpha}$ denotes $A$ for
$\alpha=1$ and $A^c$ for $\alpha=0$.

The relation $\equiv$ denotes the equality of the values of
metavariables denoting syntactic objects, so if $f_1$ and
$f_2$ are formulas, then $f_1 \equiv f_2$ means that they
are the same formula.  In the context of inclusion diagrams 
(Section~\ref{sec:idiags}),
$\equiv$ will denote the semantic equivalence of diagrams (we use
$=$ to denote the equality of diagrams).

% LocalWords:  metavariables


==> related.tex <==
\section{Related Work}

\paragraph{Boolean algebras with cardinalities.}
Quantifier-free formulas of boolean algebra are NP-complete
\cite{MarriottOdersky94NegativeBooleanConstraints}.
Quantified formulas of boolean algebra are in alternating
exponential space with a linear number of alternations
\cite{Kozen80ComplexityBooleanAlgebras}.  Cardinality
constraints naturally arise in quantifier elimination for
boolean algebras
\cite{Loewenheim15UeberMoegligkeitenRelativkalkuel,
Skolem19Untersuchungen,
Tarski49ArithmeticalClassesTypesBooleanAlgebras}.
Quantifier elimination implies that each first-order
formula of the language of boolean algebras is equivalent
to some quantifier-free formula with constant cardinalities;
however, quantifier elimination may introduce an exponential
blowup.  The first-order theory of boolean algebras of
finite sets with symbolic cardinalities, or, equivalently,
boolean algebras of sets with equicardinality operator is
shown decidable in
\cite{FefermanVaught59FirstOrderPropertiesProductsAlgebraicSystems}.
These results are repeated, motivated by constraint solving
applications, in
\cite{KuncakRinard04FirstOrderTheorySetsCardinalityConstraintsDecidable,
Revesz04QuantifierEliminationFirstOrderTheory} and a special
case with quantification over elements only is presented in
\cite{Zarba04QuantifierEliminationAlgorithmSetCardinality}.
Upper and lower bounds on the complexity of this problem were
shown in \cite{KuncakETAL05AlgorithmDecidingBAPA} which also
introduces the name $\BAPA$, for Boolean Algebra with
Presburger Arithmetic.  The quantifier-free case of $\BAPA$
was studied in \cite{Zarba05CombiningSetsCardinals} with an
NEXPTIME decision procedure, which is also achieved as a
special case of
\cite{KuncakRinard04FirstOrderTheorySetsCardinalityConstraintsDecidable,
KuncakETAL05AlgorithmDecidingBAPA}.  The new decision
procedure in the present paper improves this bound to PSPACE
and gives insight into the problem by reducing it to boolean
algebras with binary-encoded large cardinalities, and
showing that it is not necessary to explicitly construct all
set partitions.  

Several decidable fragments of set theory are studied in
\cite{CantoneETAL01SetTheoryComputing}.
Cardinality
constraints also occur in description logics
\cite{BaaderETAL03DescriptionLogicHandbook} and two-variable
logic with counting
\cite{PacholskiETAL00ComplexityResultsFirstOrderTwo,
GraedelETAL97TwoVariableLogicCountingDecidable,
PrattHartmann04CountingQuantifiersStellarFragment}.  However,
all logics of counting that we are aware of have complexity
that is beyond PSPACE.

We are not aware of any previously known fragments of boolean algebras
of sets with cardinality constraints that have polynomial-time
satisfiability or subsumption algorithms.  Our polynomial-time result
for i-trees is even more interesting in the light of the fact that our
constraints can express some ``disjunction-like'' properties such as
$A=B \cup C$.

\paragraph{Set constraints.}  Set constraints 
\cite{Aiken99SetConstraintsIntro,
AikenETAL95DecidabilitySetConstraints,
AikenETAL93ComplexitySetConstraints,
BachmairETAL93SetConstraintsMonadicClass} are incomparable
to the constraints studied in our paper.  On the one hand, set
constraints are interpreted over ground terms and contain
operations that apply a given free function symbol to each
element of the set, which makes them suitable for encoding
type inference \cite{AikenWimmers93ConstraintsTypeInference} 
and interprocedural analysis \cite{KodumalAiken04SetConstraintCFLReachabilityConnection, 
MelskiReps00InterconvertibilitySetConstraintsCFLReachability}.
Researchers have also explored the efficient computation of the subset relation for 
set constraints \cite{FaehndrichETAL98PartialOnlineCycleEliminationInclusionConstraintGraphs}.
On the
other hand, set constraints do not support cardinality
operators that are useful in modelling databases
\cite{RumbaughETAL99UMLReference,
Chen76EntityRelationshipModel} and analysis of the sizes of data
structures
\cite{LamETAL05GeneralizedTypestateCheckingDataStructureConsistency}.
Tarskian constraints use uninterpreted function symbols
instead of free function symbols and have very high
complexity \cite{GivanETAL02TarskianSetConstraints}.

% \paragraph{Linear integer constraints.}  
% The decidability of fully quantified Presburger arithmetic was shown
% in
% \cite{Presburger29UeberVollstaendigkeitSystemsAritmethikZahlen}.
% The best known
% bound on formula size is 
% \cite{FerranteRackoff79ComputationalComplexityLogicalTheories}.
% Conjunctions of linear constraints are studied in integer
% linear programming
% \cite{Schrijver98TheoryLinearIntegerProgramming}.  The
% NP-completeness of integer linear programming
% \cite{Papadimitriou81ComplexityIntegerProgramming} implies
% NP-completeness of quantifier-free Presburger arithmetic.

% LocalWords:  Skolem Tarski ArithmeticalClassesTypesBooleanAlgebras Revesz
% LocalWords:  equicardinality Presburger NEXPTIME KuncakETAL PSPACE AikenETAL
% LocalWords:  GraedelETAL PrattHartmann CountingQuantifiersStellarFragment
% LocalWords:  subsumption ComplexitySetConstraints BachmairETAL MelskiReps
% LocalWords:  SetConstraintsMonadicClass interprocedural Tarskian

